Investigating the Interplay between Spin-Polarization and Magnetic Damping in $\mathrm{Co}_{x}\mathrm{Fe}_{80-x}\mathrm{B}_{20}$ for Magnonics Applications

For magnonics and spintronics applications, the spin polarization ($P$) of a transport current and the magnetic damping ($\alpha$) play a crucial role, e.g. for magnetization dynamics and magnetization switching applications. In particular, $P$ in a glassy (amorphous) 3d transition ferromagnet such as CoFeB and $\alpha$ are both strongly affected by $s-d$ scattering mechanisms. Hence, a correlation can be expected which is a priori difficult to predict. In this work, $P$ and $\alpha$ are measured using current-induced Doppler shifts using propagating spin-wave spectroscopy and broadband ferromagnetic resonance techniques in blanket films and current-carrying $Co_{\rm x}Fe_{\rm {80-x}}B_{\rm 20}$ alloy microstrips. The measured $P$ ranges from 0.18 $\pm$ 0.05 to 0.39 $\pm$ 0.05 and $\alpha$ ranges from $(4.0\pm 0.2)\cdot10^{-3}$ to $(9.7\pm 0.6)\cdot10^{-3}$. We find that for increasing $P$ a systematic drop in $\alpha$ is observed, indicating an interplay between magnetic damping and the spin polarization of the transport current which suggests that interband scattering dominates in $Co_{\rm x}Fe_{\rm {80-x}}B_{\rm 20}$. Our results may guide future experiments, theory, and applications in advancing spintronics and metal magnonics.

==> aiptemplate.tex <==
%% ****** Start of file aiptemplate.tex ****** %
%%
%%   This file is part of the files in the distribution of AIP substyles for REVTeX4.
%%   Version 4.1 of 9 October 2009.
%%
%
% This is a template for producing documents for use with 
% the REVTEX 4.1 document class and the AIP substyles.
% 
% Copy this file to another name and then work on that file.
% That way, you always have this original template file to use.

% \documentclass[aip,graphicx]{revtex4-1}
%\documentclass[aip,reprint]{revtex4-1}

\draft % marks overfull lines with a black rule on the right

\begin{document}

% Use the \preprint command to place your local institutional report number 
% on the title page in preprint mode.
% Multiple \preprint commands are allowed.
%\preprint{}

\title{} %Title of paper

% repeat the \author .. \affiliation  etc. as needed
% \email, \thanks, \homepage, \altaffiliation all apply to the current author.
% Explanatory text should go in the []'s, 
% actual e-mail address or url should go in the {}'s for \email and \homepage.
% Please use the appropriate macro for the type of information

% \affiliation command applies to all authors since the last \affiliation command. 
% The \affiliation command should follow the other information.

\author{}
%\email[]{Your e-mail address}
%\homepage[]{Your web page}
%\thanks{}
%\altaffiliation{}
\affiliation{}

% Collaboration name, if desired (requires use of superscriptaddress option in \documentclass). 
% \noaffiliation is required (may also be used with the \author command).
%\collaboration{}
%\noaffiliation

\date{\today}

\begin{abstract}
% insert abstract here
\end{abstract}

\pacs{}% insert suggested PACS numbers in braces on next line

\maketitle %\maketitle must follow title, authors, abstract and \pacs

% Body of paper goes here. Use proper sectioning commands. 
% References should be done using the \cite, \ref, and \label commands
\section{}
%\label{}
\subsection{}
\subsubsection{}

% If in two-column mode, this environment will change to single-column format so that long equations can be displayed. 
% Use only when necessary.
%\begin{widetext}
%$$\mbox{put long equation here}$$
%\end{widetext}

% Figures should be put into the text as floats. 
% Use the graphics or graphicx packages (distributed with LaTeX2e).
% See the LaTeX Graphics Companion by Michel Goosens, Sebastian Rahtz, and Frank Mittelbach for examples. 
%
% Here is an example of the general form of a figure:
% Fill in the caption in the braces of the \caption{} command. 
% Put the label that you will use with \ref{} command in the braces of the \label{} command.
%
% \begin{figure}
% \includegraphics{}%
% \caption{\label{}}%
% \end{figure}

% Tables may be be put in the text as floats.
% Here is an example of the general form of a table:
% Fill in the caption in the braces of the \caption{} command. Put the label
% that you will use with \ref{} command in the braces of the \label{} command.
% Insert the column specifiers (l, r, c, d, etc.) in the empty braces of the
% \begin{tabular}{} command.
%
% \begin{table}
% \caption{\label{} }
% \begin{tabular}{}
% \end{tabular}
% \end{table}

% If you have acknowledgments, this puts in the proper section head.
%\begin{acknowledgments}
% Put your acknowledgments here.
%\end{acknowledgments}

% Create the reference section using BibTeX:
\bibliography{your-bib-file}

\end{document}
%
% ****** End of file aiptemplate.tex ******
